Infographics Wizard: Flexible Infographics Authoring and Design Exploration

Infographics are an aesthetic visual representation of information following specific design principles of human perception. Designing infographics can be a tedious process for non-experts and time-consuming, even for professional designers. With the help of designers, we propose a semi-automated infographic framework for general structured and flow-based infographic design generation. For novice designers, our framework automatically creates and ranks infographic designs for a user-provided text with no requirement for design input. However, expert designers can still provide custom design inputs to customize the infographics. We will also contribute an individual visual group (VG) designs dataset (in SVG), along with a 1k complete infographic image dataset with segmented VGs in this work. Evaluation results confirm that by using our framework, designers from all expertise levels can generate generic infographic designs faster than existing methods while maintaining the same quality as hand-designed infographics templates.

==> paper_files/survey.tex <==
\section{Infographics Generation Framework}



\subsection{Formative Study}
\label{ss:survey}


\begin{figure}[tb]
 \centering
 \includegraphics[width=\columnwidth]{figures/study_vg_dataset}
 \caption{\textbf{(A)} Design components of an infographic: \textit{D1} is the Visual Information Flow (VIF) layout, \textit{D2} is the Visual Group (VG) design, \textit{D3} is the pivot graphic, and \textit{D4} are the connecting elements. \textbf{(B)} Individual components inside a VG. \textbf{(C)} Example of segmented VGs in our infographics dataset. Each VG and their individual graphic elements are segmented by human annotators.}
 \label{fig:study_vg_dataset}
\end{figure}

To systematically evolve our idea of an infographic generation framework, we first conducted a formative study to get to know designers' requirements, their views of infographic designs, and general workflows. %we applied Munzner's nested model \cite{munzner2009nested,meyer2012four} similar Tyagi \textit{et al.}'s work \cite{tyagi2019ice} for visualization framework design. 
This approach helped concertize our framework and tool design with a user-centered evaluation at an earlier development stage. 
\jian{Note I removed the reference to the nested model because we did not evaluate the system at multiple levels, at least not clear. I think this is an over claim.}

The formative study participants were carefully chosen to be designers and researchers working in data visualization and infographic design, with various levels of experience. Out of ten participants, two were professional designers working in the industry, two were professors working in data visualization, three were Ph.D. students working in data visualization, and three were undergraduate students in Computer Science interested in information visualization.

The participants were initially introduced to infographics and the target we try to achieve. We asked how they would conceptually model infographic designs. Next, they were introduced to the concepts of the VIF and VG, followed by discussions about existing infographic generation tools and their shortcomings. 
We further inquired how they would use the exiting tools to design infographics and the ideal tools that they could imagine to have. 
This helped us devise a new framework that could flexibly support automated infographic generation and recommendation for various cases. %while still providing designers with the option to control the design with necessary feedback.

\subsection{Key Design Components}

Based on the study, we reconfirmed the importance of the VIF and VG concepts proposed in Lu \textit{et al.}' work \cite{lu2020exploring}.
We further consolidated four design components through designing a new framework, shown in Figure \ref{fig:study_vg_dataset}A. Each of the components is critical for designers to control for generating customized infographics. Various levels of controls result in a flexible workflow with fully- or semi-automated tools. The four key design components are:  


\textbf{D1: Visual Information Flow Layouts.} 
The participants confirmed that the concept of VIF reflects the backbones of the story or information that an infographic aims to express. Lu \textit{et al.} \cite{lu2020exploring} discovered 12 common VIF layouts. Participants further agreed that allowing designers to optionally control the VIF layout in an intuitive manner is an essential component of any infographic generation workflows. 


\textbf{D2: Visual Groups Designs.} 
The concept of VG was also echoed by the participants, and they stated that VGs could be designed separately and reused in one or multiple infographics. These VGs could then be placed according to the VIF to generate an infographic. 
They also mentioned that it is important to mitigate the effort in VG design for novices while allowing them to fully control the content of VGs and the overall structure of an infographic. The participants further mentioned that an interface separating the content and the design, like CSS and HTML for web design, could be of great benefits.  

\textbf{D3: Pivot Graphics.} 
The participants pointed out that some infographics contain a pivot graphic, which are design elements different from VGs, acting as a central background component or binding anchor for an infographic. This coincided with the ``main body'' of timeline infographics in Chen \textit{et al.}'s analysis \cite{chen2019towards}. Participants observed that such pivot graphics exist in a wide range of infograhics in addition to timelines, and stated that supporting the customization of this element is needed in infograhics design when appropriate .

\textbf{D4: Connecting Elements.} 
The participants formulated the connections between VGs, sometimes between a pivot graphic and different VGs, as one of the key infographics components. The connecting elements cannot be included into VGs because they are decorations not contributing to the content semantics of the VGs and sometimes there are no one-to-one mapping between the connections and the VGs. 
To support infographic generation, we categorized the connecting elements into three classes: regular, alternating, and pivot connections, based on our discussion with the participants (see Section \ref{s:connection} for details).


